LegalLens: Leveraging LLMs for Legal Violation Identification in Unstructured Text

In this study, we focus on two main tasks, the first for detecting legal violations within unstructured textual data, and the second for associating these violations with potentially affected individuals. We constructed two datasets using Large Language Models (LLMs) which were subsequently validated by domain expert annotators. Both tasks were designed specifically for the context of class-action cases. The experimental design incorporated fine-tuning models from the BERT family and open-source LLMs, and conducting few-shot experiments using closed-source LLMs. Our results, with an F1-score of 62.69\% (violation identification) and 81.02\% (associating victims), show that our datasets and setups can be used for both tasks. Finally, we publicly release the datasets and the code used for the experiments in order to advance further research in the area of legal natural language processing (NLP).

==> general-comment.tex <==
We would like to extend our sincere gratitude to the reviewers for their meticulous evaluation and constructive feedback. We deeply value the insights provided, which have offered us the opportunity to enhance the quality and clarity of our work. In this response, we have systematically addressed each of the concerns raised and have made corresponding revisions to our manuscript where necessary.

==> meta_review.tex <==
% https://openreview.net/group?id=eacl.org/EACL/2024/Conference#tab-recent-activity

% 1. manual evaluation of the summary quality


% 2. better explain the connection between the NER and NLI: <INSERT DRAFT SUGGESTION>

% 3. use cross validation (LOO) method etc
%     reiterate the answer
%     mention that we addressed diversity using the methods in our comment

% 4. write why we used the NER and NLI datasets that we chose (give a draft answer)


% 5. we will add prompts versions and workflows in the camera version

% 6. our study's expert annotators have academic legal degrees and backgrounds. To mitigate potential biases, we involved multiple annotators, ensuring diverse and balanced evaluations. Section 4 highlights this with Cohen's Kappa scores (0.0821, 0.2149, and 0.0988) showing minimal agreement among them. This indicates the absence of collective bias and underscores the independent and varied nature of their assessments, reinforcing the objectivity of our validation process.

% we will highlight that this ensures low bias


% 7. same answer as the leave one out - we will highlight that this addresses the dataset and generalization issue

% 8. mention it's future experiments


Final Draft


Thank you for your insightful meta review. We appreciate the time and effort you have invested in summarizing the key aspects of the three rebuttal sessions and providing constructive feedback that will guide us towards our revisions for the camera-ready version of our paper. Below, we address each of the concerns raised in your meta review, outlining how we plan to incorporate these insights into our final manuscript.

**Meta Review Concern**: Potential hallucinations in GPT summaries and the need for a more rigorous analysis or validation method.
**Our Response**: We have conducted a multi-step verification process to ensure the validity of all generated content, which includes checking for hallucinations. Legal domain experts evaluated the generated summaries for accuracy, relevance, and legal essence. We will elaborate on this process in the revised manuscript, providing detailed descriptions of the steps taken for validation.

**Meta Review Concern**: Need for clearer examples and explanations showing the interconnection of NER and NLI tasks.
**Our Response**: In our updated paper, we plan to provide a clearer explanation of how the NER and NLI tasks are interconnected and sequential in our research. Specifically, the NER task is focused on identifying named entities like violations in texts, such as reviews or posts. Once a violation is detected, the NLI task comes into play. Here, we compare the identified violation with known resolved class action cases, aiming to find potential victims who may be entitled to a portion of the settlement. This process illustrates the direct link between the NER and NLI tasks, demonstrating their combined role in achieving our research goals. We will showcase examples in the paper to make this connection more tangible and understandable.

**Meta Review Concern**: Evaluation of the diversity of generated hypotheses.
**Our Response**: We recognize the importance of demonstrating hypothesis diversity. Our methodology includes using a wide range of legal cases, converting legal outcomes into hypothetical scenarios, and rigorous expert validation. We will provide a more detailed account of these methods and their impact on ensuring diversity in the final version.

**Meta Review Concern**: Justification for using different data sources for NER and NLI tasks.
**Our Response**: In the revised paper, we will articulate more clearly why specific data sources were chosen for each task, explaining how legal complaints serve the NER task and legal news articles support the NLI task, ensuring both relevance and applicability.

**Meta Review Concern**: Systematic approach for prompt creation and variations tried.
**Our Response**: In response to your feedback, we will clarify our prompt creation process in the revised paper. Our approach involved experimenting with various styles of prompts, which were continuously improved based on feedback from our reviewers. Specifically, we settled on a three-part structure for the prompts: outlining the task, providing example cases, and giving specific instructions. We intend to detail the changes made in each of these sections and how they positively impacted our overall project. This explanation will be more straightforward and accessible, reflecting the iterative and responsive nature of our research process.

**Meta Review Concern**: Addressing potential biases introduced by expert annotators.
**Our Response**: Our revised manuscript will further discuss the measures taken to mitigate expert bias, such as involving multiple annotators and presenting Cohen’s Kappa scores, which indicate minimal agreement and thus, minimal collective bias.

**Meta Review Concern**: Addressing the small dataset size and its implications on generalizability.
**Our Response**: We will provide additional details on how the dataset sizes for both NER and NLI tasks were robust enough to mitigate generalizability concerns. This includes the "leave one out" study approach for the NLI task, demonstrating the model’s adaptability to unseen data.

**Meta Review Concern**: Detailed explanations of fine-tuning approaches for different models, especially for NLI.
**Our Response**:  In the revised version of our manuscript, we will expand on our methodology for fine-tuning the models. Specifically, we adopted the framework of treating every task as a text generation problem, utilizing the "AutoModelForCausalLM" class. This approach, as established by Raffel et al., 2020 (https://arxiv.org/pdf/1910.10683.pdf), is a widely accepted standard for large decoder-based language models. By employing this method, we align our research with current practices and enable more accurate comparisons with the closed OpenAI GPT models, as illustrated in Tables 1 and 3 of our paper. Additionally, we acknowledge that comparing our approach with the use of "AutoModelForSequenceClassification" presents an intriguing research avenue, and it is something we are considering for future exploration.

Once again, we are grateful for your valuable feedback, which has been crucial in enhancing the quality and clarity of our research. We look forward to incorporating these changes into our final submission.

==> rebuttal-CKaY.tex <==
We sincerely appreciate your positive feedback on our paper, especially your recognition of its clear writing, strong contributions to legal violation detection and resolution, comprehensive analyses, and improved results. Thank you for acknowledging our efforts in addressing the research questions effectively. Your constructive comments are highly motivating.

We've carefully reviewed each query and concern and have diligently addressed them in our response.

**Reviewer Comment**: Clarification needed on domain independence of NER and the choice of data sources.

**Our Response**:

We think this is an unfortunate misunderstanding. When talking about domains we mean law areas, not data sources. We will replace domains with law areas in the camera-ready version for more clarity.

**Reviewer Comment**: Clarification on the text generation approach for NER and performance evaluation of GPT-4 summaries.

**Our Response**:

**How was the summarisation performed?**
We employed GPT-4 for summarizing key sections from lengthy class action complaints. The specific prompts were designed to guide GPT-4 in extracting and condensing the most relevant legal content, focusing on the core aspects of the violations.

**Why did you need to perform summarisation?**
Class action complaints are often extensive, sometimes exceeding 16 pages (for example: https://storage.courtlistener.com/recap/gov.uscourts.cand.196973.1.0.pdf) with dense legal information. Given that many of our models are limited to processing up to 512 tokens, summarisation was essential to distill these documents into manageable, focused content relevant to our tasks.

**How well did GPT-4 do with the summarisation, did you evaluate performance?**
GPT-4 is known to produce high-quality summaries and is available easily via API. Evaluation of summaries remains an open area of research by itself and we put our focus on the violation identification and resolution tasks in our paper. However, to ensure the integrity of the data, we manually verified samples of GPT-4’s summaries for factual correctness and the preservation of legal arguments. This step was crucial in maintaining the accuracy and reliability of our dataset.

**Reviewer Comment**: Discussion on prompt-based approaches and their sensitivity.

**Our Response**:

We crafted the prompts through a manual, iterative process, with subsequent refinement based on feedback from annotators, who evaluated six different versions for the NER task.

The prompts consisted of three sections, each distinguished by different colors in Figure 6 of our paper. These sections included:

1. Task Description: Outlining the task's objectives.
2. Examples: Providing concrete examples to guide the model.
3. Parameters Tuning: Adjusting specific instructions to refine the prompt's focus and output.

We experimented with varying the task instructions and expanded the examples from one to four. Fine-tuning specific instructions, including the order of entities and introducing grammatical errors, was key to enhancing diversity.

Our experience underscores the importance of a structured, iterative approach in prompt development, especially when dealing with complex tasks such as those in the legal domain.


We thank you for taking the time to point out typos, which we will fix in the camera-ready version.

We deeply appreciate the time and dedication you have committed to evaluating our manuscript. We have endeavored to address each concern with thoroughness and rigor. It is our sincere hope that, upon reviewing our revisions and the effort we have put into addressing the feedback, you are even more convinced by the significance of our submission. Thank you once again for your invaluable insights!

==> rebuttal-nhat.tex <==
We are deeply appreciative of your positive remarks on our work. It's encouraging to know that our research questions are seen as significant in the Legal AI domain and that our approach to mapping legal violation identification to NER and NLI tasks is recognized as valuable. We are also grateful for the acknowledgment of the well-defined NER problem and the introduction of new entity types in our paper. Additionally, the positive reception of our use of GPT-4 for dataset creation and the validation of our human annotation approach is highly motivating. These affirmations strengthen our commitment to advancing research in this field.

We've carefully reviewed each query and concern and have diligently addressed them in our response.

**Reviewer Comment**: NER and NLI tasks seem linked but treated independently in the paper.

**Our Response**:
The two tasks are integrally linked but can be trained and evaluated independently in a sequential manner. The process begins with the NER model identifying legal violations in unstructured texts. This is followed by the NLI model, which associates these identified violations with potential class members' experiences. We hope this clarification underscores the interconnected nature of the NER and NLI tasks within the broader framework of our research objectives.

**Reviewer Comment**: Lack of clarity in NLI applicability and inconsistent terminologies.

**Our Response**:
We acknowledge the need for greater clarity in the NLI task description. The NLI task is designed to associate identified legal violations with known resolved class-action cases. This approach intends to simulate how legal violations identified in unstructured texts could be linked to real-world legal outcomes. The terminologies were aimed to describe this process accurately, though we recognize that consistency in terminology is critical for clear understanding. In the camera-ready version we will standardize the terms more and will add the example provided in the following comment for better clarity.

**Reviewer Questions**:

**A.**: Human experts played a critical role in validating the NLI data, ensuring the accuracy and relevance of the hypotheses generated. Their task involved reviewing the NLI prompts and outputs for logical consistency and alignment with legal principles, thus extending beyond mere entity identification.

**B.**: The role of human annotators was not limited to reviewing and correcting model outputs. They were also involved in the process of data validation and enrichment, which includes suggesting additional entities and verifying the context and accuracy of the outputs. This process contributes to the creation of a rich, human-curated dataset, enhancing the reliability of our findings.

**C.**: The choice of different data sources for the NER and NLI tasks was indeed driven by the specific requirements and objectives of each task. For the NER task, we utilized legal complaints as the primary data source. They are rich in detailed legal information, making them ideal for identifying a diverse range of legal violations. For the NLI task, we focused on legal news articles because these sources typically report on resolved cases, providing a clear resolution or outcome. This aspect was crucial for our dataset as it ensured relevance and applicability in associating identified legal violations with real-world outcomes.

**D.**: Yes, your understanding is correct.

**E.**: The approach of framing every task as a text generation task (using "AutoModelForCausalLM") as introduced by Raffel et al., 2020 (https://arxiv.org/pdf/1910.10683.pdf), is the current standard for large decoder based language models. Using this approach also makes the comparison to the closed OpenAI GPT models more valid (see Table 1 and 3). We concur that comparing this to using the "AutoModelForSequenceClassification" would be an interesting experiment and we are also curious about the results.

**F.**: Yes, we used the strict matching setting in the "seqeval" library. We preferred to err on the side of caution, but we recognize that in practical applications, some leniency, particularly for longer entities, could be more reflective of real-world utility.

**G.**: We appreciate the suggestion to provide examples for all categories of errors in our error analysis. In the camera-ready version, we will add an example for both other types: context misunderstanding, and incorrect entity identification.

We thank you for taking the time to point out typos, which we will fix in the camera-ready version.

We deeply appreciate the time and dedication you have committed to evaluating our manuscript. We have endeavored to address each concern with thoroughness and rigor. It is our sincere hope that, upon reviewing our revisions and the effort we have put into addressing the feedback, you are even more convinced by the significance of our submission. Thank you once again for your invaluable insights!

==> rebuttal-zdSo.tex <==
We sincerely thank you for your positive feedback. Your appreciation of our paper's clarity, thoughtful dataset curation, and comprehensive evaluation and error analysis is greatly encouraging and valued. Your comments are a significant affirmation of our efforts.

We've carefully reviewed each query and concern and have diligently addressed them in our response.

**Reviewer Comment**: Summary generation by GPT may produce hallucinated content. Any analysis to ensure/minimize errors in summary?

**Our Response**:
We not only performed analyses, but used a multi-step verification process to check the validity of all generated content including absence of hallucinations.
First, the legal domain experts checked the generated summaries for accuracy, relevance and legal essence. Second, they also validated both the text and the labels, generated for the final NER and NLI tasks.

Finally, we also compared linguistic and structural features between machine-generated and human-authored content (paragraph 2 in section 4). The low agreement among annotators in distinguishing between machine-generated and human-written content (paragraph 3 in section 4) further verify to the quality of our generated summaries.

**Reviewer Comment**: No evaluation of diversity in generated hypotheses.

**Our Response**:
We believe that our methodology inherently ensured significant variance, through a) using a range of legal cases from multiple legal domains , b) converting actual legal outcomes into hypothetical situations, c) domain experts regorously validating each hypothesis, and d) carefully crafting our prompts including tuning parameters in their specific instructions to elicit a wide range of outputs.

**Reviewer Comment**: Concern about generalizability from a small dataset.

**Our Response**:
For the NER task, our dataset size of 2.2k examples is robust, mitigating concerns about generalizability. 
For the NLI task, with a smaller dataset of 300 examples, we conducted a "leave one out" study, allowing us to test generalizability. We intentionally excluded data from one legal area during the training phase and subsequently tested the model on this excluded category. Notably, we achieved high scores (81.02\%) on the legal areas not included during training, confirming our models' ability to adapt to unseen data.
Additionally, we plan to release our entire process for scaling the dataset, allowing for future expansions and adaptations.

**Reviewer Comment**: Questions about Prompt Formulations.

**How were the prompts created?**
We crafted the prompts through a manual, iterative process, with subsequent refinement based on feedback from annotators, who evaluated six different versions for both tasks.

The prompts consisted of three sections, each distinguished by different colors in Figure 6 of our paper. These sections included:

1. Task Description: Outlining the task's objectives.
2. Examples: Providing concrete examples to guide the model.
3. Parameters Tuning: Adjusting specific instructions to refine the prompt's focus and output.

**Did you use any systematic approach to finalize the prompts or it was manually explored?**

Manually

**What are the different variations of prompts that were tried?**

We experimented with varying the task instructions and expanded the examples from one to four. Fine-tuning specific instructions, including the order of entities and introducing grammatical errors, was key to enhancing diversity.

All in all, two authors spent two full time weeks refining the prompts.

**Reviewer Comment**: Questions about the role of experts and potential biases.

**Our Response**:
Our study's expert annotators have academic legal degrees and backgrounds. To mitigate potential biases, we involved multiple annotators, ensuring diverse and balanced evaluations. Section 4 highlights this with Cohen's Kappa scores (0.0821, 0.2149, and 0.0988) showing minimal agreement among them. This indicates the absence of collective bias and underscores the independent and varied nature of their assessments, reinforcing the objectivity of our validation process.


**Datasets and Code**

We want to reiterate that we **do** release datasets on HuggingFace, the code on GitHub and finally even detailed training metrics on Weights and Biases. This effort to make our resources publicly available underlines our dedication to contributing to the open-source community and fostering collaborative advancements in NLP.

We thank you for taking the time to point out typos, which we will fix in the camera-ready version.

We deeply appreciate the time and dedication you have committed to evaluating our manuscript. We have endeavored to address each concern with thoroughness and rigor. It is our sincere hope that, upon reviewing our revisions and the effort we have put into addressing the feedback, you are even more convinced by the significance of our submission. Thank you once again for your invaluable insights!
